Full-Body Torque-Level Non-linear Model Predictive Control for Aerial Manipulation

Non-linear model predictive control (nMPC) is a powerful approach to control complex robots (such as humanoids, quadrupeds, or unmanned aerial manipulators (UAMs)) as it brings important advantages over other existing techniques. The full-body dynamics, along with the prediction capability of the optimal control problem (OCP) solved at the core of the controller, allows to actuate the robot in line with its dynamics. This fact enhances the robot capabilities and allows, e.g., to perform intricate maneuvers at high dynamics while optimizing the amount of energy used. Despite the many similarities between humanoids or quadrupeds and UAMs, full-body torque-level nMPC has rarely been applied to UAMs. This paper provides a thorough description of how to use such techniques in the field of aerial manipulation. We give a detailed explanation of the different parts involved in the OCP, from the UAM dynamical model to the residuals in the cost function. We develop and compare three different nMPC controllers: Weighted MPC, Rail MPC, and Carrot MPC, which differ on the structure of their OCPs and on how these are updated at every time step. To validate the proposed framework, we present a wide variety of simulated case studies. First, we evaluate the trajectory generation problem, i.e., optimal control problems solved offline, involving different kinds of motions (e.g., aggressive maneuvers or contact locomotion) for different types of UAMs. Then, we assess the performance of the three nMPC controllers, i.e., closed-loop controllers solved online, through a variety of realistic simulations. For the benefit of the community, we have made available the source code related to this work.

==> sections/introduction_old.tex <==
% !TEX root =  ../root.tex


\section{Introduction} \label{sec:introduction}
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/cover.pdf}\vspace{-0.em}
  \caption{Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption Caption }
  \label{fig:cover}
\end{figure}

An \gls{am} is pretty much like a humanoid. 
They both have arms, bla bla ...

\phtopic{UAM concept introduction}
Aerial robots were initially conceived as flying sensor suites and, therefore, they were used in missions involving only data collection and its treatment (\eg, filming, surveillance or mapping).
Naturally, the need for interaction with the environment emerged, fostering the appearance of \glspl*{am}. %different robots and applications.
The range of complexity of \glspl*{am} is wide, from a flying platform with a rigidly attached gripper for object transportation, to a more complex fully-actuated multi-rotor endorsed with several articulated arms~\cite{ruggiero_am_literature_review_2018,khamseh_am_survey_2018}.

\phtopic{Traditional PL/Ctrl algs simplify models}
Current state-of-the-art planning and control algorithms for \glspl*{am} often involve the analytical manipulation of the kinematic or dynamic expressions.
This is a quite involving procedure for single rigid body systems (multicopters) and its difficulty considerably increases when we attach articulated bodies to the platform.
This is a quite involving procedure for single rigid body systems (multicopters).
The difficulty of this procedure increases with the attachment of other articulated bodies to the platform.
In this case, to reduce the complexity and still be able to manage the expressions, it is common to do some simplifications.
These, use to affect either the modelling of the problem or the robot (sometimes both), keeping the formulation tractable.

\phtopic{Traditional Ctrl: decentralized}
The traditional algorithms devoted to control this kind of robots was exported from the respective individual subsystems, on the one hand from single multicopters and on the other hand from fixed-base manipulators.
This has led to \emph{decentralized} approaches, which aim at controlling independently the flying base and the robotic arm~\cite{ruggiero_multilayer_2015}.
Due to this decentralization, the coupling forces at the union of both robots are considered to be disturbances for the respective controllers.
Big forces may also cause stability issues to the platform and, seeking to minimize them, the \gls*{am} tends to move in a quasi-static manner (\eg\ roll and pitch angles are assumed to be zero by the arm controller).
A typical scheme for a decentralized approach is to consider a motion planner at the kinematic level, which normally resolves the kinematic redundancy of the \gls*{am}~\cite{rossi_trajgeneration_2017,lipiello_visualservoing_2016}.
This outputs separated position set-points for the controllers of the platform and the arm.
Eventually, the planner sends conservative commands not only to minimize the interaction force but also to ensure that each controller reaches the desired positions within the required time.

\phtopic{Intro to centralized Ctrl: feedback linearization}
Contrarily, \emph{centralized} approaches consider the full-body \gls*{am} dynamics, hence coping with the coupled dynamics.
Among these, a common choice is to apply feedback linearization.
Its application slightly varies depending on the actuated \glspl*{dof} of the platform.
Using fully actuated platforms (like the one presented in~\cite{rajappa_tilthex_2015}) allows for their full-translational control, and the outputs selected to apply this technique are the linear and angular velocities of the platform along with the joint velocities of the arm~\cite{tognon_control-aware_2018}.
When dealing with under-actuated platforms, we should carefully choose the outputs for feedback linearization.
In~\cite{kim_stabilizing_2018}, the choice is the linear velocity along the vertical axis of the platform, its orientation and the joint velocities of the arm.
Anyhow, once the outputs are selected, applying feedback linearization to a system results in a feedback control law depending on a desired acceleration, which can be properly shaped to render the system stable.
Having this kind of control is powerful since its feedback law cancels the dynamics of the system and thus eases the shaping of the state evolution.
However, the ability to cancel the dynamics comes at the price of high control commands and therefore rough movements.

\phtopic{Centralized Ctrl: differential flatness}
A similar idea to feedback linearization is the so-called \emph{differential flatness}.
Differential flatness is a property of a system that allows us to express the states and inputs as a function of several outputs and their higher order derivatives. These are the so-called \emph{flat outputs}.
This eases the planning phase since we only need to generate a trajectory for the flat outputs and retrieve automatically the control inputs.
Finding the equations that relate states and inputs to the flat outputs involves manipulating the equations of the dynamics of the system.
In aerial robotics, differential flatness was first used for simple multicopter-based systems.
For example, in~\cite{mellinger_minimum_2011} the set of flat outputs for a multicopter is constituted by its center of mass position and the yaw angle.
In similar systems, like a quadcopter with a cable-suspended load~\cite{sreenath_cablesuspended_2013}, the flat outputs are the position of the suspended mass and the yaw angle of the quadcopter.
When the complexity of the system increases, which is the case of \glspl*{am}, finding deferentially flat outputs becomes a difficult task.
In \cite{yuksel_differential_2016,tognon_dynamic_2017} it is shown how the center of mass of the platform together with the absolute orientation angles of all the links of the arm constitute a set of flat outputs.
However, this only holds if the first joint of the arm coincides with the center of mass of the platform.
Moreover, the arm is restricted to be planar, \ie, all the axes of the joints should be parallel, which severely limits its practical interest. 

\phtopic{Intro to interaction ENV and what others proposed}
Any \gls*{am} control technique should enable a fundamental capability: the interaction with the environment.
In~\cite{ryll_6dinteraction_2019}, they consider a fully actuated hexacopter with a rigidly attached end-effector to solve several problems involving a physical interaction.
The contact and the force applied to the surface is indirectly handled by setting desired positions of the end-effector.
By means of an admittance filter, they compute a reference for the hexacopter's geometric controller.
In~\cite{hamaza_adaptivecompliance_2018}, it is proposed a \gls*{am} design with a 1-\gls*{dof} arm to apply a force to a specific point.
In~\cite{tognon_trulyredundant_2019}, a fully actuated platform with a 2-\gls*{dof} arm is used to perform a "push \& slide" maneuver in a cylindrical surface.
They propose a custom PID controller to overcome the hardware limitations (velocity-controlled joints and link flexibility).
However, the interactions considered in all these approaches is limited either to simplistic operations or to the application of forces on surfaces~\cite{kondak_uasinteraction_2015}.
For instance, the idea of using the contact as a source of motion (\ie, the contact-locomotion for \gls*{am}) has been rarely explored and, to the best of the authors' knowledge, there exists only one reference exploring this path,~\cite{delamare_toward_2018}, with a simplified 2D model of an \gls*{am} (\eg, with a 1-\gls*{dof} arm) hanging from a bar that is able to jump to another bar by exploiting the gripping contact.

\phtopic{What else has not been covered to interact with ENV}
In addition to the idea of contact-locomotion for \glspl*{am}, there are other scenarios involving aerial manipulation that are strangely covered in the literature.
These include, for instance, aggressive maneuvers with complex \glspl*{am} or changes in the robot model during flight operations due to, \eg, a change in its mass (typical from pick and place operations).
 

\subsection{Similarities with legged robots}
\phtopic{Intro why leggeds are interesting}
The desire of having complex robots performing fast and agile movements that eventually might involve contacts with the environment is not new to the robotics community.
In fact, these are the standard requirements for %those working with 
\emph{legged robots}, for which contacts are inherent and represent the only means of motion generation.
Within this community, finding techniques to produce aggressive movements has been a hot topic in recent years, \eg~\cite{mastalli_hierarchical_2016,park_highspeed_cheetah_2017}.
Given the similarity between legged systems and \glspl*{am} (both are underactuated devices with a floating base with several kinematic chains attached to it)\footnote{Taking this similarity to the limit, one could think that attaching some propellers to the torso of a humanoid allowing it to fly, would convert this robot into a \gls*{am}.}, we believe that some of the techniques used in the former devices can be imported into the aerial manipulation field with the aim of enhancing \glspl*{am}' capabilities.

\phtopic{What we want to take to UAMs}
Specifically, we want to pay attention to the way of planning motions and, eventually, control the legged robot to execute the movement.
Formerly, the problem of legged locomotion was solved by breaking it down to a cascade of sub-problems to, eventually, send the commands to the actuators.
In particular, given a predefined contact sequence, they solved a hierarchical \gls*{ik} followed by an \gls*{id}, producing directly the torque commands to the actuators~\cite{saab_dynamic_wholebody_2013}.
Nowadays, the community is leaning to consider full-body \glspl*{ocp} (\cite{betts_practicalmethods_optimalcontrol_book}), which allows to unify the planning and control phases~\cite{rawlings_modelpredictivecontrol_book,koenemann_wholebody_2015,neunert_wholebody_2018}.
Moreover, these techniques allow for a better modelling of the system and its constraints~\cite{budhiraja_ddp_multiphase_2018}, which leads to improved movements.

\phtopic{Philosophical contribution}
In this paper, we leverage the experience from the legged robots' community and propose the use of optimal control as a framework to tackle all potential applications for aerial manipulators within a unified and generic control approach.

\subsection{Optimal control \& aerial robotics}
\phtopic{We want to use MPC}
There have been several works where optimal control has been applied to aerial manipulation.
Either solving the \gls*{ocp} online to control the robot using \gls*{nmpc} techniques, or offline as a trajectory generator.
In~\cite{lunni_nonlinear_2017}, it is proposed an \gls*{nmpc} controller at a kinematic level to generate set points for a low-level controller in a decentralized architecture.
A closer approach to our current proposal can be found in~\cite{garimella_towards_2015,geisert_trajectory_2016}.
Even though they consider the full-body dynamics, both use \gls*{ocp} to generate a trajectory but not to control the \gls*{am} with an \gls*{nmpc} controller.
Besides, none of them consider contacts.
In~\cite{tzoumanikas_aerial_2020}, they present a hybrid-\gls*{nmpc} to perform a writing task with a delta robot.
That is, the \gls*{ocp} in the controller solves the problem at a force level for the platform and at the position level for the end-effector of the robotic arm.
Besides, the dynamical model is simplified by considering quasi-static maneuvers.

\phtopic{methods using full-body nMPC}
To the best of the authors' knowledge, full body \gls*{nmpc} at the force/torque level has not been proposed for \glspl*{am}.
However, there have been a few proposals involving single multicopters.
In~\cite{kamel_fastnonlinear_2015}, they use a \gls*{nmpc} controller to track the attitude given by a higher level trajectory generator.
An improved version is shown in~\cite{neunert_fast_2016}, where they unify the planning an the control block.
They use a \gls*{slq} solver to solve, online, an \gls*{ocp} and apply the optimized thrust commands to the motors.
Even though it is not very clear from the paper, it seems from the formulation that waypoints out of the controller horizon are treated following a \gls*{nmpc} approach (see \secref{sec:mpc}).
A similar approach is taken in~\cite{brunner_trajectory_2020}, where they consider the omnidirectional multicopter described in~\cite{brescianini_omni_2016}.
They use the derivative of the wrench on the body as the control variable in the \gls*{nmpc}.
Afterwards, they perform the control allocation to retrieve the rotor speed and tilt angles.

\subsection{Contribution \& Paper outline}

\phtopic{Contributions}
\label{sec:contribution}
The main contributions of this work include:
\begin{enumerate}
  \item A generic framework that allows us to consider a wide variety of \glspl*{am} (\ie, diverse multicopter platforms and manipulators). Our numerical approach to the problem allows to change the \gls*{am} with a small overhead on the modeling side.
  \item The possibility to generate fast and agile maneuvers with complex \glspl*{am} thanks to a full-body \gls*{ocp} that we solve online to send commands to the actuators at the force/torque level.
  \item The consideration of multiphase problems, involving contacts that may favor the robot's motion (resembling the locomotion in legged robots).
  \item We can consider problems that involve changes in the parameters of the robot's dynamical equation during the mission. For instance, this allows us to model a change in the mass of the end-effector, typical of "pick \& place" operations.
  \item We present clear developments and compare different strategies to transition from an \gls*{ocp} used for planning to an \gls*{ocp} used for control (\gls*{nmpc}).
  \item All the software tools used to conduct the presented experiments in \secref{sec:validation} are made available for the benefit of the community.
\end{enumerate}

\phtopic{Table Of Contents}
The rest of the paper is structured as follows.
In \secref{sec:optimal_control}, we first give a brief overview of the existing manners to solve an \gls*{ocp} to eventually, explain the method that we use, which is an improved version of \gls*{ddp}.
The following sections are devoted to explain the formulation of the several parts involved in the \gls*{ocp}.
First, in \secref{sec:modeling}, we explain how we build the dynamical model of a robot with branched connectivity when is moving freely through the space or is in contact with the environment.
Also in this section, we explain how to consider any kind of multicopter platform with fixed propeller orientation.
Second, in \secref{sec:cost_functions} we show how we build the cost function talking about its structure as well as the different residuals contained in it.
In \secref{sec:mpc}, we present different strategies to move from the \gls*{ocp} used to generate trajectories offline (\ie, planning), to \gls*{ocp}s used to control robots.
The stated contributions are finally tested in different experiments in \secref{sec:validation}. First, we present a set of several maneuvers involving complex situations. These are solved offline to generate a trajectory. Second, we compare the performance of different \gls*{nmpc} techniques for different kind of maneuvers and \gls*{am}.
The application of optimal control techniques in \gls*{am} involve some challenges that are not solved yet.
We give an overview in the concluding remarks in \secref{sec:conclusions}.

